An Abstract Framework for Choreographic Testing

We initiate the development of a model-driven testing framework for message-passing systems. The notion of test for communicating systems cannot simply be borrowed from existing proposals. Therefore, we formalize a notion of suitable distributed tests for a given choreography and devise an algorithm that generates tests as projections of global views. Our algorithm abstracts away from the actual projection operation, for which we only set basic requirements. The algorithm can be instantiated by reusing existing projection operations (designed to generate local implementations of global models) as they satisfy our requirements. Finally, we show the correctness of the approach and validate our methodology via an illustrative example.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{J. Lange, A. Mavridou, L. Safina, A. Scalas (Eds.):\\
13th Interaction and Concurrency Experience (ICE 2020).\\
EPTCS 324, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.324.5}{10.4204/EPTCS.324.5}}
\pdfoutput=1


==> main-dot2tex-fig1.tex <==
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \definecolor{fillcol}{rgb}{1.0,1.0,1.0};
  \pgfsetfillcolor{fillcol}
  \filldraw (0.0bp,0.0bp) -- (0.0bp,419.0bp) -- (822.0bp,419.0bp) -- (822.0bp,0.0bp) -- cycle;
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,137.0bp) -- (814.0bp,137.0bp) -- (814.0bp,8.0bp) -- cycle;
  \draw (411.0bp,125.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,137.0bp) -- (814.0bp,137.0bp) -- (814.0bp,8.0bp) -- cycle;
  \draw (411.0bp,125.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,145.0bp) -- (8.0bp,274.0bp) -- (814.0bp,274.0bp) -- (814.0bp,145.0bp) -- cycle;
  \draw (411.0bp,262.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,145.0bp) -- (8.0bp,274.0bp) -- (814.0bp,274.0bp) -- (814.0bp,145.0bp) -- cycle;
  \draw (411.0bp,262.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,282.0bp) -- (8.0bp,411.0bp) -- (814.0bp,411.0bp) -- (814.0bp,282.0bp) -- cycle;
  \draw (411.0bp,399.5bp) node {ATM Machine};
\end{scope}
  \node (C1) at (229.0bp,42.0bp) [draw,ellipse] {C1};
  \node (B1) at (229.0bp,179.0bp) [draw,ellipse] {B1};
  \node (A2) at (229.0bp,335.0bp) [draw,ellipse] {A2};
  \node (C4) at (615.0bp,88.0bp) [draw,ellipse] {C4};
  \coordinate (Co) at (779.0bp,88.0bp);
  \coordinate (C0) at (43.0bp,42.0bp);
  \node (C2) at (449.0bp,42.0bp) [draw,ellipse] {C2};
  \node (C3) at (615.0bp,34.0bp) [draw,ellipse] {C3};
  \node (B4) at (615.0bp,225.0bp) [draw,ellipse] {B4};
  \coordinate (Bo) at (779.0bp,225.0bp);
  \coordinate (B0) at (43.0bp,179.0bp);
  \node (B2) at (449.0bp,179.0bp) [draw,ellipse] {B2};
  \node (B3) at (615.0bp,171.0bp) [draw,ellipse] {B3};
  \node (A1) at (43.0bp,335.0bp) [draw,ellipse] {A1};
  \node (A3) at (449.0bp,335.0bp) [draw,ellipse] {A3};
  \node (A4) at (615.0bp,308.0bp) [draw,ellipse] {A4};
  \node (A6) at (615.0bp,362.0bp) [draw,ellipse] {A6};
  \node (A5) at (779.0bp,308.0bp) [draw,ellipse] {A5};
  \node (A7) at (779.0bp,362.0bp) [draw,ellipse] {A7};
  \draw [->] (C1) ..controls (295.11bp,42.0bp) and (367.86bp,42.0bp)  .. (C2);
  \draw (339.0bp,49.5bp) node {CA!withdraw};
  \draw [->] (C2) ..controls (503.38bp,39.396bp) and (546.73bp,37.281bp)  .. (C3);
  \draw (532.0bp,46.5bp) node {AC?bye};
  \draw [->] (C2) ..controls (479.49bp,53.247bp) and (487.0bp,55.86bp)  .. (494.0bp,58.0bp) .. controls (522.39bp,66.685bp) and (555.11bp,74.739bp)  .. (C4);
  \draw (532.0bp,84.5bp) node {AC?money};
  \draw [->] (B1) ..controls (295.11bp,179.0bp) and (367.86bp,179.0bp)  .. (B2);
  \draw (339.0bp,186.5bp) node {AB?authWithdraw};
  \draw [->] (B2) ..controls (503.38bp,176.4bp) and (546.73bp,174.28bp)  .. (B3);
  \draw (532.0bp,183.5bp) node {BA!deny};
  \draw [->] (B2) ..controls (479.49bp,190.25bp) and (487.0bp,192.86bp)  .. (494.0bp,195.0bp) .. controls (522.39bp,203.68bp) and (555.11bp,211.74bp)  .. (B4);
  \draw (532.0bp,221.5bp) node {BA!allow};
  \draw [->] (A1) ..controls (102.29bp,335.0bp) and (156.22bp,335.0bp)  .. (A2);
  \draw (136.0bp,342.5bp) node {CA?withdraw};
  \draw [->] (A2) ..controls (295.11bp,335.0bp) and (367.86bp,335.0bp)  .. (A3);
  \draw (339.0bp,342.5bp) node {AB!authWithdraw};
  \draw [->] (A3) ..controls (479.74bp,324.57bp) and (487.1bp,322.46bp)  .. (494.0bp,321.0bp) .. controls (521.86bp,315.12bp) and (553.96bp,311.82bp)  .. (A4);
  \draw (532.0bp,328.5bp) node {BA?deny};
  \draw [->] (A3) ..controls (503.31bp,343.78bp) and (547.6bp,351.07bp)  .. (A6);
  \draw (532.0bp,361.5bp) node {BA?allow};
  \draw [->] (A4) ..controls (668.99bp,308.0bp) and (711.34bp,308.0bp)  .. (A5);
  \draw (697.0bp,315.5bp) node {AC!bye};
  \draw [->] (A6) ..controls (668.99bp,362.0bp) and (711.34bp,362.0bp)  .. (A7);
  \draw (697.0bp,369.5bp) node {AC!money};
%

==> main-dot2tex-fig2.tex <==
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,191.0bp) -- (1069.0bp,191.0bp) -- (1069.0bp,8.0bp) -- cycle;
  \draw (538.5bp,179.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,191.0bp) -- (1069.0bp,191.0bp) -- (1069.0bp,8.0bp) -- cycle;
  \draw (538.5bp,179.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,191.0bp) -- (1069.0bp,191.0bp) -- (1069.0bp,8.0bp) -- cycle;
  \draw (538.5bp,179.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,191.0bp) -- (1069.0bp,191.0bp) -- (1069.0bp,8.0bp) -- cycle;
  \draw (538.5bp,179.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,191.0bp) -- (1069.0bp,191.0bp) -- (1069.0bp,8.0bp) -- cycle;
  \draw (538.5bp,179.5bp) node {Client Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,199.0bp) -- (8.0bp,382.0bp) -- (1069.0bp,382.0bp) -- (1069.0bp,199.0bp) -- cycle;
  \draw (538.5bp,370.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,199.0bp) -- (8.0bp,382.0bp) -- (1069.0bp,382.0bp) -- (1069.0bp,199.0bp) -- cycle;
  \draw (538.5bp,370.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,199.0bp) -- (8.0bp,382.0bp) -- (1069.0bp,382.0bp) -- (1069.0bp,199.0bp) -- cycle;
  \draw (538.5bp,370.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,199.0bp) -- (8.0bp,382.0bp) -- (1069.0bp,382.0bp) -- (1069.0bp,199.0bp) -- cycle;
  \draw (538.5bp,370.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,199.0bp) -- (8.0bp,382.0bp) -- (1069.0bp,382.0bp) -- (1069.0bp,199.0bp) -- cycle;
  \draw (538.5bp,370.5bp) node {Bank Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,390.0bp) -- (8.0bp,627.0bp) -- (1069.0bp,627.0bp) -- (1069.0bp,390.0bp) -- cycle;
  \draw (538.5bp,615.5bp) node {ATM Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,390.0bp) -- (8.0bp,627.0bp) -- (1069.0bp,627.0bp) -- (1069.0bp,390.0bp) -- cycle;
  \draw (538.5bp,615.5bp) node {ATM Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,390.0bp) -- (8.0bp,627.0bp) -- (1069.0bp,627.0bp) -- (1069.0bp,390.0bp) -- cycle;
  \draw (538.5bp,615.5bp) node {ATM Machine};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,390.0bp) -- (8.0bp,627.0bp) -- (1069.0bp,627.0bp) -- (1069.0bp,390.0bp) -- cycle;
  \draw (538.5bp,615.5bp) node {ATM Machine};
\end{scope}
  \node (C3) at (467.0bp,34.0bp) [draw,circle, double] {};
  \node (C6) at (687.0bp,88.0bp) [draw,circle, double] {};
  \node (C8) at (862.0bp,34.0bp) [draw,circle, double] {};
  \node (C9) at (862.0bp,88.0bp) [draw,circle, double] {};
  \node (C10) at (862.0bp,142.0bp) [draw,circle, double] {};
  \coordinate (Co) at (1034.0bp,142.0bp);
  \node (C4) at (467.0bp,88.0bp) [draw,fill=red,ellipse] {};
  \node (C7) at (687.0bp,142.0bp) [draw,fill=lightgray,ellipse] {};
  \node (C1) at (43.0bp,61.0bp) [draw,ellipse] {};
  \node (C2) at (236.5bp,61.0bp) [draw,ellipse] {};
  \node (C5) at (687.0bp,34.0bp) [draw,ellipse] {};
  \node (B3) at (467.0bp,225.0bp) [draw,circle, double] {};
  \node (B10) at (687.0bp,333.0bp) [draw,circle, double] {};
  \node (B6) at (862.0bp,225.0bp) [draw,circle, double] {};
  \node (B7) at (862.0bp,279.0bp) [draw,circle, double] {};
  \node (B9) at (862.0bp,333.0bp) [draw,circle, double] {};
  \node (B2) at (236.5bp,252.0bp) [draw,fill=red,ellipse] {};
  \node (B5) at (687.0bp,225.0bp) [draw,fill=red,ellipse] {};
  \coordinate (Bo) at (1034.0bp,333.0bp);
  \node (B8) at (687.0bp,279.0bp) [draw,fill=lightgray,ellipse] {};
  \node (B1) at (43.0bp,252.0bp) [draw,ellipse] {};
  \node (B4) at (467.0bp,279.0bp) [draw,ellipse] {};
  \node (A1) at (43.0bp,578.0bp) [draw,ellipse] {};
  \node (A6) at (43.0bp,506.0bp) [draw,ellipse] {};
  \node (A5) at (862.0bp,578.0bp) [draw,circle, double] {};
  \node (A11) at (1034.0bp,524.0bp) [draw,circle, double] {};
  \node (A13) at (1034.0bp,470.0bp) [draw,circle, double] {};
  \node (A15) at (687.0bp,416.0bp) [draw,circle, double] {};
  \node (A19) at (1034.0bp,416.0bp) [draw,circle, double] {};
  \node (A4) at (687.0bp,578.0bp) [draw,fill=lightgray,ellipse] {};
  \node (A14) at (467.0bp,416.0bp) [draw,fill=lightgray,ellipse] {};
  \node (A16) at (467.0bp,470.0bp) [draw,fill=lightgray,ellipse] {};
  \node (A10) at (862.0bp,524.0bp) [draw,fill=lightgray,ellipse] {};
  \node (A12) at (862.0bp,470.0bp) [draw,fill=lightgray,ellipse] {};
  \node (A2) at (236.5bp,578.0bp) [draw,ellipse] {};
  \node (A3) at (467.0bp,578.0bp) [draw,ellipse] {};
  \node (A7) at (236.5bp,470.0bp) [draw,ellipse] {};
  \node (A8) at (467.0bp,524.0bp) [draw,ellipse] {};
  \node (A9) at (687.0bp,524.0bp) [draw,ellipse] {};
  \node (A17) at (687.0bp,470.0bp) [draw,ellipse] {};
  \node (A18) at (862.0bp,416.0bp) [draw,ellipse] {};
  \draw [->] (C1) ..controls (103.65bp,61.0bp) and (161.61bp,61.0bp)  .. (C2);
  \draw (132.0bp,68.5bp) node {CA!auth};
  \draw [->] (C2) ..controls (272.4bp,51.73bp) and (285.26bp,48.822bp)  .. (297.0bp,47.0bp) .. controls (342.46bp,39.947bp) and (395.42bp,36.66bp)  .. (C3);
  \draw (359.5bp,54.5bp) node {AC?authFail};
  \draw [->] (C2) ..controls (304.09bp,68.868bp) and (383.74bp,78.28bp)  .. (C4);
  \draw (359.5bp,89.5bp) node {AC?granted};
  \draw [->] (C4) ..controls (496.62bp,74.516bp) and (504.54bp,71.334bp)  .. (512.0bp,69.0bp) .. controls (558.84bp,54.353bp) and (614.75bp,44.383bp)  .. (C5);
  \draw (577.0bp,76.5bp) node {CA!withdraw};
  \draw [->] (C4) ..controls (533.11bp,88.0bp) and (605.86bp,88.0bp)  .. (C6);
  \draw (577.0bp,95.5bp) node {CA!quit};
  \draw [->] (C4) ..controls (496.62bp,101.48bp) and (504.54bp,104.67bp)  .. (512.0bp,107.0bp) .. controls (558.84bp,121.65bp) and (614.75bp,131.62bp)  .. (C7);
  \draw (577.0bp,142.5bp) node {CA!checkBalance};
  \draw [->] (C5) ..controls (743.7bp,34.0bp) and (791.59bp,34.0bp)  .. (C8);
  \draw (774.5bp,41.5bp) node {AC?bye};
  \draw [->] (C5) ..controls (716.72bp,47.172bp) and (724.62bp,50.419bp)  .. (732.0bp,53.0bp) .. controls (763.33bp,63.951bp) and (799.91bp,73.59bp)  .. (C9);
  \draw (774.5bp,84.5bp) node {AC?money};
  \draw [->] (C7) ..controls (743.7bp,142.0bp) and (791.59bp,142.0bp)  .. (C10);
  \draw (774.5bp,149.5bp) node {AC?balance};
  \draw [->] (B1) ..controls (103.65bp,252.0bp) and (161.61bp,252.0bp)  .. (B2);
  \draw (132.0bp,259.5bp) node {AB?authReq};
  \draw [->] (B2) ..controls (272.4bp,242.73bp) and (285.26bp,239.82bp)  .. (297.0bp,238.0bp) .. controls (342.46bp,230.95bp) and (395.42bp,227.66bp)  .. (B3);
  \draw (359.5bp,245.5bp) node {BA!denied};
  \draw [->] (B2) ..controls (304.09bp,259.87bp) and (383.74bp,269.28bp)  .. (B4);
  \draw (359.5bp,280.5bp) node {BA!granted};
  \draw [->] (B4) ..controls (496.62bp,265.52bp) and (504.54bp,262.33bp)  .. (512.0bp,260.0bp) .. controls (558.84bp,245.35bp) and (614.75bp,235.38bp)  .. (B5);
  \draw (577.0bp,267.5bp) node {AB?authWithdraw};
  \draw [->] (B4) ..controls (533.11bp,279.0bp) and (605.86bp,279.0bp)  .. (B8);
  \draw (577.0bp,286.5bp) node {AB?getBalance};
  \draw [->] (B4) ..controls (496.62bp,292.48bp) and (504.54bp,295.67bp)  .. (512.0bp,298.0bp) .. controls (558.84bp,312.65bp) and (614.75bp,322.62bp)  .. (B10);
  \draw (577.0bp,333.5bp) node {AB?quit};
  \draw [->] (B5) ..controls (743.7bp,225.0bp) and (791.59bp,225.0bp)  .. (B6);
  \draw (774.5bp,232.5bp) node {BA!deny};
  \draw [->] (B5) ..controls (716.72bp,238.17bp) and (724.62bp,241.42bp)  .. (732.0bp,244.0bp) .. controls (763.33bp,254.95bp) and (799.91bp,264.59bp)  .. (B7);
  \draw (774.5bp,275.5bp) node {BA!allow};
  \draw [->] (B8) ..controls (741.63bp,295.74bp) and (793.35bp,311.88bp)  .. (B9);
  \draw (774.5bp,325.5bp) node {BA!balance};
  \draw [->] (A1) ..controls (103.65bp,578.0bp) and (161.61bp,578.0bp)  .. (A2);
  \draw (132.0bp,585.5bp) node {CA?auth};
  \draw [->] (A2) ..controls (304.49bp,578.0bp) and (383.25bp,578.0bp)  .. (A3);
  \draw (359.5bp,585.5bp) node {AB!authReq};
  \draw [->] (A3) ..controls (533.11bp,578.0bp) and (605.86bp,578.0bp)  .. (A4);
  \draw (577.0bp,585.5bp) node {BA?denied};
  \draw [->] (A3) ..controls (406.16bp,562.43bp) and (337.94bp,545.67bp)  .. (279.0bp,536.0bp) .. controls (194.77bp,522.18bp) and (172.21bp,529.93bp)  .. (88.0bp,516.0bp) .. controls (84.93bp,515.49bp) and (81.754bp,514.9bp)  .. (A6);
  \draw (236.5bp,543.5bp) node {BA?granted};
  \draw [->] (A4) ..controls (743.7bp,578.0bp) and (791.59bp,578.0bp)  .. (A5);
  \draw (774.5bp,585.5bp) node {AC!authFail};
  \draw [->] (A6) ..controls (103.0bp,494.91bp) and (162.28bp,483.76bp)  .. (A7);
  \draw (132.0bp,504.5bp) node {AC!granted};
  \draw [->] (A7) ..controls (272.75bp,478.63bp) and (285.47bp,481.58bp)  .. (297.0bp,484.0bp) .. controls (352.29bp,495.58bp) and (367.64bp,491.64bp)  .. (422.0bp,507.0bp) .. controls (426.08bp,508.15bp) and (430.31bp,509.53bp)  .. (A8);
  \draw (359.5bp,514.5bp) node {CA?withdraw};
  \draw [->] (A7) ..controls (271.14bp,457.05bp) and (284.63bp,452.37bp)  .. (297.0bp,449.0bp) .. controls (342.48bp,436.61bp) and (396.05bp,426.96bp)  .. (A14);
  \draw (359.5bp,456.5bp) node {CA?quit};
  \draw [->] (A7) ..controls (273.97bp,469.28bp) and (286.05bp,469.09bp)  .. (297.0bp,469.0bp) .. controls (352.55bp,468.53bp) and (366.45bp,468.37bp)  .. (422.0bp,469.0bp) .. controls (424.54bp,469.03bp) and (427.16bp,469.07bp)  .. (A16);
  \draw (359.5bp,476.5bp) node {CA?checkBalance};
  \draw [->] (A8) ..controls (533.11bp,524.0bp) and (605.86bp,524.0bp)  .. (A9);
  \draw (577.0bp,531.5bp) node {AB!authWithdraw};
  \draw [->] (A14) ..controls (533.11bp,416.0bp) and (605.86bp,416.0bp)  .. (A15);
  \draw (577.0bp,423.5bp) node {AB!quit};
  \draw [->] (A16) ..controls (533.11bp,470.0bp) and (605.86bp,470.0bp)  .. (A17);
  \draw (577.0bp,477.5bp) node {AB!getBalance};
  \draw [->] (A9) ..controls (743.7bp,524.0bp) and (791.59bp,524.0bp)  .. (A10);
  \draw (774.5bp,531.5bp) node {BA?deny};
  \draw [->] (A9) ..controls (716.72bp,510.83bp) and (724.62bp,507.58bp)  .. (732.0bp,505.0bp) .. controls (763.33bp,494.05bp) and (799.91bp,484.41bp)  .. (A12);
  \draw (774.5bp,512.5bp) node {BA?allow};
  \draw [->] (A10) ..controls (917.89bp,524.0bp) and (964.14bp,524.0bp)  .. (A11);
  \draw (948.0bp,531.5bp) node {AC!bye};
  \draw [->] (A12) ..controls (917.89bp,470.0bp) and (964.14bp,470.0bp)  .. (A13);
  \draw (948.0bp,477.5bp) node {AC!money};
  \draw [->] (A17) ..controls (741.63bp,453.26bp) and (793.35bp,437.12bp)  .. (A18);
  \draw (774.5bp,462.5bp) node {BA?balance};
  \draw [->] (A18) ..controls (917.89bp,416.0bp) and (964.14bp,416.0bp)  .. (A19);
  \draw (948.0bp,423.5bp) node {AC!balance};
%

==> main-dot2tex-fig3.tex <==
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,91.0bp) -- (821.0bp,91.0bp) -- (821.0bp,8.0bp) -- cycle;
  \draw (414.5bp,79.5bp) node {M-Bank 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,91.0bp) -- (821.0bp,91.0bp) -- (821.0bp,8.0bp) -- cycle;
  \draw (414.5bp,79.5bp) node {M-Bank 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,91.0bp) -- (821.0bp,91.0bp) -- (821.0bp,8.0bp) -- cycle;
  \draw (414.5bp,79.5bp) node {M-Bank 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,91.0bp) -- (821.0bp,91.0bp) -- (821.0bp,8.0bp) -- cycle;
  \draw (414.5bp,79.5bp) node {M-Bank 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,99.0bp) -- (8.0bp,228.0bp) -- (821.0bp,228.0bp) -- (821.0bp,99.0bp) -- cycle;
  \draw (414.5bp,216.5bp) node {M-Bank 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,99.0bp) -- (8.0bp,228.0bp) -- (821.0bp,228.0bp) -- (821.0bp,99.0bp) -- cycle;
  \draw (414.5bp,216.5bp) node {M-Bank 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,99.0bp) -- (8.0bp,228.0bp) -- (821.0bp,228.0bp) -- (821.0bp,99.0bp) -- cycle;
  \draw (414.5bp,216.5bp) node {M-Bank 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,236.0bp) -- (8.0bp,365.0bp) -- (821.0bp,365.0bp) -- (821.0bp,236.0bp) -- cycle;
  \draw (414.5bp,353.5bp) node {M-Bank 1};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,236.0bp) -- (8.0bp,365.0bp) -- (821.0bp,365.0bp) -- (821.0bp,236.0bp) -- cycle;
  \draw (414.5bp,353.5bp) node {M-Bank 1};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,236.0bp) -- (8.0bp,365.0bp) -- (821.0bp,365.0bp) -- (821.0bp,236.0bp) -- cycle;
  \draw (414.5bp,353.5bp) node {M-Bank 1};
\end{scope}
  \node (Ba3) at (394.0bp,38.0bp) [draw,fill=lightgray,circle, double] {};
  \coordinate (Ba4) at (614.0bp,38.0bp);
  \coordinate (Ba5) at (786.0bp,38.0bp);
  \node (Ba1) at (43.0bp,38.0bp) [draw,ellipse] {};
  \node (Ba2) at (221.0bp,38.0bp) [draw,ellipse] {};
  \node (Bc6) at (786.0bp,125.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Bc9) at (786.0bp,179.0bp) [draw,circle, double] {};
  \node (Bc8) at (614.0bp,179.0bp) [draw,fill=lightgray,ellipse] {};
  \node (Bc1) at (43.0bp,152.0bp) [draw,ellipse] {};
  \node (Bc2) at (221.0bp,152.0bp) [draw,ellipse] {};
  \node (Bc4) at (394.0bp,152.0bp) [draw,ellipse] {};
  \node (Bc5) at (614.0bp,125.0bp) [draw,ellipse] {};
  \node (Bd7) at (786.0bp,262.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Bd9) at (786.0bp,316.0bp) [draw,circle, double] {};
  \node (Bd8) at (614.0bp,316.0bp) [draw,fill=lightgray,ellipse] {};
  \node (Bd1) at (43.0bp,289.0bp) [draw,ellipse] {};
  \node (Bd2) at (221.0bp,289.0bp) [draw,ellipse] {};
  \node (Bd4) at (394.0bp,289.0bp) [draw,ellipse] {};
  \node (Bd5) at (614.0bp,262.0bp) [draw,ellipse] {};
  \draw [->] (Ba1) ..controls (100.37bp,38.0bp) and (149.64bp,38.0bp)  .. (Ba2);
  \draw (132.0bp,45.5bp) node {AB?authReq};
  \draw [->] (Ba2) ..controls (278.81bp,38.0bp) and (328.94bp,38.0bp)  .. (Ba3);
  \draw (307.5bp,45.5bp) node {BA!denied};
  \draw [->] (Bc1) ..controls (100.37bp,152.0bp) and (149.64bp,152.0bp)  .. (Bc2);
  \draw (132.0bp,159.5bp) node {AB?authReq};
  \draw [->] (Bc2) ..controls (277.3bp,152.0bp) and (324.01bp,152.0bp)  .. (Bc4);
  \draw (307.5bp,159.5bp) node {BA!granted};
  \draw [->] (Bc4) ..controls (424.71bp,141.41bp) and (432.07bp,139.34bp)  .. (439.0bp,138.0bp) .. controls (485.9bp,128.92bp) and (541.04bp,126.09bp)  .. (Bc5);
  \draw (504.0bp,145.5bp) node {AB?authWithdraw};
  \draw [->] (Bc4) ..controls (459.71bp,160.01bp) and (533.22bp,169.12bp)  .. (Bc8);
  \draw (504.0bp,180.5bp) node {AB?getBalance};
  \draw [->] (Bc5) ..controls (669.89bp,125.0bp) and (716.14bp,125.0bp)  .. (Bc6);
  \draw (700.0bp,132.5bp) node {BA!deny};
  \draw [->] (Bc8) ..controls (669.89bp,179.0bp) and (716.14bp,179.0bp)  .. (Bc9);
  \draw (700.0bp,186.5bp) node {BA!balance};
  \draw [->] (Bd1) ..controls (100.37bp,289.0bp) and (149.64bp,289.0bp)  .. (Bd2);
  \draw (132.0bp,296.5bp) node {AB?authReq};
  \draw [->] (Bd2) ..controls (277.3bp,289.0bp) and (324.01bp,289.0bp)  .. (Bd4);
  \draw (307.5bp,296.5bp) node {BA!granted};
  \draw [->] (Bd4) ..controls (424.71bp,278.41bp) and (432.07bp,276.34bp)  .. (439.0bp,275.0bp) .. controls (485.9bp,265.92bp) and (541.04bp,263.09bp)  .. (Bd5);
  \draw (504.0bp,282.5bp) node {AB?authWithdraw};
  \draw [->] (Bd4) ..controls (459.71bp,297.01bp) and (533.22bp,306.12bp)  .. (Bd8);
  \draw (504.0bp,317.5bp) node {AB?getBalance};
  \draw [->] (Bd5) ..controls (669.89bp,262.0bp) and (716.14bp,262.0bp)  .. (Bd7);
  \draw (700.0bp,269.5bp) node {BA!allow};
  \draw [->] (Bd8) ..controls (669.89bp,316.0bp) and (716.14bp,316.0bp)  .. (Bd9);
  \draw (700.0bp,323.5bp) node {BA!balance};
%

==> main-dot2tex-fig4.tex <==
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \definecolor{fillcol}{rgb}{1.0,1.0,1.0};
  \pgfsetfillcolor{fillcol}
  \filldraw (0.0bp,0.0bp) -- (0.0bp,419.0bp) -- (798.0bp,419.0bp) -- (798.0bp,0.0bp) -- cycle;
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \definecolor{fillcol}{rgb}{1.0,1.0,1.0};
  \pgfsetfillcolor{fillcol}
  \filldraw (0.0bp,0.0bp) -- (0.0bp,419.0bp) -- (798.0bp,419.0bp) -- (798.0bp,0.0bp) -- cycle;
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,137.0bp) -- (790.0bp,137.0bp) -- (790.0bp,8.0bp) -- cycle;
  \draw (399.0bp,125.5bp) node {M-Client 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,137.0bp) -- (790.0bp,137.0bp) -- (790.0bp,8.0bp) -- cycle;
  \draw (399.0bp,125.5bp) node {M-Client 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,8.0bp) -- (8.0bp,137.0bp) -- (790.0bp,137.0bp) -- (790.0bp,8.0bp) -- cycle;
  \draw (399.0bp,125.5bp) node {M-Client 3};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,145.0bp) -- (8.0bp,274.0bp) -- (790.0bp,274.0bp) -- (790.0bp,145.0bp) -- cycle;
  \draw (399.0bp,262.5bp) node {M-Client 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,145.0bp) -- (8.0bp,274.0bp) -- (790.0bp,274.0bp) -- (790.0bp,145.0bp) -- cycle;
  \draw (399.0bp,262.5bp) node {M-Client 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,145.0bp) -- (8.0bp,274.0bp) -- (790.0bp,274.0bp) -- (790.0bp,145.0bp) -- cycle;
  \draw (399.0bp,262.5bp) node {M-Client 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,145.0bp) -- (8.0bp,274.0bp) -- (790.0bp,274.0bp) -- (790.0bp,145.0bp) -- cycle;
  \draw (399.0bp,262.5bp) node {M-Client 2};
\end{scope}
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (8.0bp,282.0bp) -- (8.0bp,411.0bp) -- (790.0bp,411.0bp) -- (790.0bp,282.0bp) -- cycle;
  \draw (399.0bp,399.5bp) node {M-Client 1};
\end{scope}
  \node (Cc3) at (368.0bp,308.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Cc10) at (755.0bp,362.0bp) [draw,circle, double] {};
  \node (Cc7) at (582.0bp,362.0bp) [draw,fill=lightgray,ellipse] {};
  \node (Ca3) at (368.0bp,34.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Ca8) at (755.0bp,34.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Ca9) at (755.0bp,88.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Ca1) at (43.0bp,63.0bp) [draw,ellipse] {};
  \node (Ca2) at (192.0bp,63.0bp) [draw,ellipse] {};
  \node (Ca4) at (368.0bp,88.0bp) [draw,ellipse] {};
  \node (Ca5) at (582.0bp,88.0bp) [draw,ellipse] {};
  \node (Cb3) at (368.0bp,171.0bp) [draw,fill=lightgray,circle, double] {};
  \node (Cb6) at (582.0bp,225.0bp) [draw,fill=lightgray,circle, double] {};
  \coordinate (Co) at (755.0bp,225.0bp);
  \node (Cb1) at (43.0bp,198.0bp) [draw,ellipse] {};
  \node (Cb2) at (192.0bp,198.0bp) [draw,ellipse] {};
  \node (Cb4) at (368.0bp,225.0bp) [draw,ellipse] {};
  \node (Cc1) at (43.0bp,335.0bp) [draw,ellipse] {};
  \node (Cc2) at (192.0bp,335.0bp) [draw,ellipse] {};
  \node (Cc4) at (368.0bp,362.0bp) [draw,ellipse] {};
  \draw [->] (Ca1) ..controls (93.797bp,63.0bp) and (128.5bp,63.0bp)  .. (Ca2);
  \draw (117.5bp,70.5bp) node {CA!auth};
  \draw [->] (Ca2) ..controls (223.13bp,53.318bp) and (230.29bp,51.394bp)  .. (237.0bp,50.0bp) .. controls (268.31bp,43.494bp) and (304.45bp,39.308bp)  .. (Ca3);
  \draw (280.0bp,57.5bp) node {AC?authFail};
  \draw [->] (Ca2) ..controls (248.44bp,70.966bp) and (297.71bp,78.044bp)  .. (Ca4);
  \draw (280.0bp,88.5bp) node {AC?granted};
  \draw [->] (Ca4) ..controls (433.08bp,88.0bp) and (502.31bp,88.0bp)  .. (Ca5);
  \draw (475.0bp,95.5bp) node {CA!withdraw};
  \draw [->] (Ca5) ..controls (611.73bp,74.847bp) and (619.62bp,71.596bp)  .. (627.0bp,69.0bp) .. controls (657.72bp,58.193bp) and (693.55bp,48.581bp)  .. (Ca8);
  \draw (668.5bp,76.5bp) node {AC?bye};
  \draw [->] (Ca5) ..controls (638.3bp,88.0bp) and (685.01bp,88.0bp)  .. (Ca9);
  \draw (668.5bp,95.5bp) node {AC?money};
  \draw [->] (Cb1) ..controls (93.797bp,198.0bp) and (128.5bp,198.0bp)  .. (Cb2);
  \draw (117.5bp,205.5bp) node {CA!auth};
  \draw [->] (Cb2) ..controls (222.73bp,187.53bp) and (230.09bp,185.43bp)  .. (237.0bp,184.0bp) .. controls (268.24bp,177.54bp) and (304.38bp,174.26bp)  .. (Cb3);
  \draw (280.0bp,191.5bp) node {AC?authFail};
  \draw [->] (Cb2) ..controls (248.44bp,206.6bp) and (297.71bp,214.25bp)  .. (Cb4);
  \draw (280.0bp,224.5bp) node {AC?granted};
  \draw [->] (Cb4) ..controls (433.08bp,225.0bp) and (502.31bp,225.0bp)  .. (Cb6);
  \draw (475.0bp,232.5bp) node {CA!quit};
  \draw [->] (Cc1) ..controls (93.797bp,335.0bp) and (128.5bp,335.0bp)  .. (Cc2);
  \draw (117.5bp,342.5bp) node {CA!auth};
  \draw [->] (Cc2) ..controls (222.73bp,324.53bp) and (230.09bp,322.43bp)  .. (237.0bp,321.0bp) .. controls (268.24bp,314.54bp) and (304.38bp,311.26bp)  .. (Cc3);
  \draw (280.0bp,328.5bp) node {AC?authFail};
  \draw [->] (Cc2) ..controls (248.44bp,343.6bp) and (297.71bp,351.25bp)  .. (Cc4);
  \draw (280.0bp,361.5bp) node {AC?granted};
  \draw [->] (Cc4) ..controls (433.08bp,362.0bp) and (502.31bp,362.0bp)  .. (Cc7);
  \draw (475.0bp,369.5bp) node {CA!checkBalance};
  \draw [->] (Cc7) ..controls (638.3bp,362.0bp) and (685.01bp,362.0bp)  .. (Cc10);
  \draw (668.5bp,369.5bp) node {AC?balance};
%
